Make Text Unlearnable: Exploiting Effective Patterns to Protect Personal Data

This paper addresses the ethical concerns arising from the use of unauthorized public data in deep learning models and proposes a novel solution. Specifically, building on the work of Huang et al. (2021), we extend their bi-level optimization approach to generate unlearnable text using a gradient-based search technique. However, although effective, this approach faces practical limitations, including the requirement of batches of instances and model architecture knowledge that is not readily accessible to ordinary users with limited access to their own data. Furthermore, even with semantic-preserving constraints, unlearnable noise can alter the text's semantics. To address these challenges, we extract simple patterns from unlearnable text produced by bi-level optimization and demonstrate that the data remains unlearnable for unknown models. Additionally, these patterns are not instance- or dataset-specific, allowing users to readily apply them to text classification and question-answering tasks, even if only a small proportion of users implement them on their public content. We also open-source codes to generate unlearnable text and assess unlearnable noise to benefit the public and future studies.

==> deleted_paragraphs.tex <==
\chapter{Make Text Unlearnable}
\label{chapter:unlearnable}
\section{Prologue}
Similar to poisoning data, unlearnable examples are against training eligible models. However, they would prevent the model from learning the information instead of causing a malicious impact on the model. This is used for the unauthorized usage of users' data for training models.

\paragraph{Methodology}
This is very similar to solve the aforementioned bi-level optimization problem for data poison. The difference is that the inner objective is to perturb the input data while the outer one is for training the model. Therefore, it interests us whether unlearnable texts could be constructed by unrolling the training steps and then applying the gradient approximation to solve the inner objective.


\paragraph{Compared to the formulation from \citet{huang2021unlearnable}.}
\begin{equation}
\begin{split} 
& \text{class-wise} \\
& \quad \forall (x, y) \in \mathcal{D}, p(y|b) = p(y|b, x) \\
& \text{sample-wise} \\
& \quad \forall (x, y) \in \mathcal{D}  \exists b, p(y|b) = p(y|b, x)  \\
\end{split}
\end{equation}

We cannot ensure whether such patterns exist in the min-min noise for images, which can make data unlearnable. 
However, although we cannot find such patterns, we can directly optimize a bias feature $b$ separately during the training process rather than use bi-level optimization to generate the noise.

Therefore, the objective equals to minimize the cross-entropy loss.
\begin{equation} \label{eq:unlearnable1}
\begin{split} 
\underset{\theta}{\arg \min } \mathbf{E}_{(x+b, y) \sim \mathcal{D}}[\underset{b}{\arg \min } \mathcal{L}(f(b), y)] 
\end{split}
\end{equation}

\paragraph{Compared the semantics to protect.}
The semantics they need to prevent deep learning from exploiting are objects or humans portrayed in images, e.g., face recognition. 
In contrast, the semantics of texts are distributed across variable lengths of sequences, which further compose of discrete variables (words or characters). 

\paragraph{Callback Implementation: Text Modification Callback during Training.} 
To implement Algorithm without interfering the training process, we only provide a callback object to generate unlearnable text and modify the training data.


\paragraph{Small surrogate models for transformers.}
% problem/solution
Although the current downstream NLP models based on pre-trained transformers are often optimized via the pre-training and fine-tuning paradigm, generating effective modifications is very computationally expensive during training. In practice, due to the constraint of the computation resource, optimizating over the large pre-trained language models become more unrealistic. 
Hence, we perform the gradient-based approach on simple neural nets to explore unlearnable patterns. We assume that statistical features can be common in a architecture-invariant manner.
% in fact, generating substitutions for sub-words would be an explorable challenges for me (Plan for my next phase of research).


Neural text classification models are known to explore statistical patterns during supervised learning. However, such patterns include spurious patterns and superficial regularity in the training data. In this paper, we exaggerate superficial regularity in the text to prevent unauthorized exploration of personal data. 


Our framework also provides an theoretical testbed and explanation for the empirical conclusions of the shortcut phenomenon in previous works. \citep{branco-etal-2021-shortcutted,lai-etal-2021-machine,bai2021attention}. 
For example, according to our statistical framework, we conclude that the model achieves the highly unlearnable state once a low-entropy conditional distribution $p(y|b)$ is generated. It explains the empirical result that "the high proportions of shortcut questions in the training data may hinder the model from learning challenging skills" \citep{lai-etal-2021-machine}. Actually, "the high proportions of shortcut questions" helps achieve the unlearnable state. 
% We empirically prove these theoretical hypotheses by tracking the gradients during the training dynamics.
% Besides, the unlearnable state would not last for too many epochs.


We find that our proposed method can automatically find the easiest unlearnable patterns (Section \ref{sec:classification}): inserting simple synthetic characters (e.g., 'a', 'b', 'c') into the training data in the class-wise manner could be effective for unlearnable training, no matter where they are inserted. Such modified text has the same semantics as the original one but prevents DNNs (including pre-trained transformers) from learning transferable generalizations, i.e., causing low model performance on the test data due to unlearnable data.

\paragraph{By comparing shortcuts and optimized unlearnable biases}, we further verity that the latter can achieve the unlearnable state more quickly than the shortcuts found in previous study. 

\paragraph{Which triggers are more effective?} 
Class-wise triggers have been studied for adversarial text and are effective to cause adversarial behaviours \citep{wallace2019universal,behjati2019universal}. They find the optimal triggers for adversarial attacks via the iterative optimization. We can search optimal triggers in the unlearnable settings. To do this, we insert a words $\vect{t}$ at the beginning of each samples and then optimize $\vect{t}$. Compared to sample-wise word substitutions, we only optimize substitutions $s$ for fixed positions $p$. 
just $s$ with fixed $p$, where we insert one word $s$ in either the beginning, middle or ending of the sentence \footnote{Beginning: ${s, w_2, w_1, ..., w_{T+1} }$; \\ Middle: ${w_1, ..., s, ...w_{T+1} }$ where $s$ is inserted into the position indexed by the ceiling of $\frac{2}{T}$; \\ Ending: ${w_1, w_2, ..., w_T, s }$ }
Compared to optimize $(p, s)$, the latter one only needs to search over the vocabulary for one fixed position. 
% The result shows that arbitrarily initialized class-wise triggers can be effective, which terminates optimization at the initial stage.
% Practical: users can easily process text rather than modify each content they want to post online.

% By investigating the training process, gradient norm become zero from 200 steps (1 epoch) at the same time  the training acurracy as shown in Figure \ref{fig:grad_norm}.  indicating that the model stopped learning after correlating the class-wise triggers with the class.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{pics/grad_norm.png}
%     \caption{Change of gradient norm during training.}
%     \label{fig:grad_norm}
% \end{figure}

% \citet{huang2021unlearnable} shows that image classifiers perform with a negligible effect even when 40\% training data is transformed into unlearnable examples. 
% Detail:
% sst-calss-wise-0.8 | sst-minus-0.8unlearnable
% One curious finding: 
% the smaller the batch size is, the larger the gradient magnitudes.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\textwidth]{pics/unlearnable_percent.png}
%     \caption{}
%     \label{fig:percent}
% \end{figure}



% \paragraph{Once the model has learned the shortcut, it cannot learn anything from data with the shortcut.} 
% What it means for "has learned"? loss of any data with shortcut would be zero.
% Experiment Prove:
% We construct two unlearnable sets and two clean sets $\mathcal{D}_{u1}$, $\mathcal{D}_{u2}$, $\mathcal{D}_{c1}$ and $\mathcal{D}_{c2}$. We fine-tune the BERT using these four datasets in the order of $\mathcal{D}_{u1}$, $\mathcal{D}_{c1}$, $\mathcal{D}_{u2}$,  $\mathcal{D}_{c2}$.

% \begin{table}[ht!]
%     \centering
%     \begin{tabular}{|c|c|}
%         \hline
%          & Test accuracy \\ \hline \hline
%         $\mathcal{D}_{1}$ &0. \\ \hline
%         $\mathcal{D}_{u1}$ &0. \\ \hline
%         $\mathcal{D}_{2}$ &0. \\ \hline
%         $\mathcal{D}_{u2}$ &0. \\ \hline
%     \end{tabular}
%     \caption{}
%     \label{tab:partial}
% \end{table}

% experiment design
\paragraph{Partial unlearnable data for SQuAD.}
To avoid expensive computation, we design a different experiment to evaluate the effectiveness of partial unlearnable data for SQuAD.

We construct two sets for training $\mathcal{D}_{1}$, $\mathcal{D}_{2}$, each of which consists of 1000 samples. We protect $\mathcal{D}_{1}$ to be an unlearnable set $\mathcal{D}_{u1}$. 
% we re-use the unlearnable mdoficatoins generated from BiDAF. 
We then fine-tune the transformer with $\mathcal{D}_{u1} \cup \mathcal{D}_{2}$. 

% result
We compare the model performance on $\mathcal{D}_{1}$ and $\mathcal{D}_{2}$ to evaluate whether $\mathcal{D}_{u1}$ can protect $\mathcal{D}_{1}$. We also report unseen test data $\mathcal{D}_{test}$ as the reference. As shown in Table \ref{tab:squad_partial}, the model performs much worse on $\mathcal{D}_{u1}$ than $\mathcal{D}_{2}$. Hence, it can be effective to make partial data unlearnable for SQuAD.

% how about $\mathcal{D}_{2} \cup \mathcal{D}_{u1}$.
% how about spreading unlearnable data into each batch during training?
% What 's the threshold of effectiveness?

% clean 0.921 - 0.797
{
  "best_epoch": 2,
  "untrained_test_start_acc": 0.011,
  "untrained_test_end_acc": 0.008,
  "untrained_test_span_acc": 0.0,
  "untrained_test_per_instance_em": 0.0,
  "untrained_test_per_instance_f1": 0.034397081318034366,
  "peak_worker_0_memory_MB": 0,
  "peak_gpu_0_memory_MB": 2935.8623046875,
  "test_start_acc": 0.914,
  "test_end_acc": 0.904,
  "test_span_acc": 0.852,
  "test_per_instance_em": 0.868,
  "test_per_instance_f1": 0.9213911410939646,
  "training_duration": "0:04:06.696871",
  "epoch": 4,
  "training_start_acc": 0.844,
  "training_end_acc": 0.848,
  "training_span_acc": 0.761,
  "training_loss": 0.5353626986921188,
  "training_worker_0_memory_MB": 0.0,
  "training_gpu_0_memory_MB": 2935.8623046875,
  "validation_start_acc": 0.651,
  "validation_end_acc": 0.624,
  "validation_span_acc": 0.547,
  "validation_per_instance_em": 0.685,
  "validation_per_instance_f1": 0.7395262655832846,
  "validation_loss": 1.658784991540946,
  "best_validation_start_acc": 0.653,
  "best_validation_end_acc": 0.627,
  "best_validation_span_acc": 0.552,
  "best_validation_per_instance_em": 0.69,
  "best_validation_per_instance_f1": 0.7421301095644991,
  "best_validation_loss": 1.5885611491538585
}
% 80% unlearn span_acc  0.556-0.637 f1:0.709 - 0.797
Metrics: {
  "best_epoch": 4,
  "untrained_test_start_acc": 0.011,
  "untrained_test_end_acc": 0.008,
  "untrained_test_span_acc": 0.0,
  "untrained_test_per_instance_em": 0.0,
  "untrained_test_per_instance_f1": 0.03366374798470106,
  "peak_worker_0_memory_MB": 0,
  "peak_gpu_0_memory_MB": 3234.48095703125,
  "test_start_acc": 0.633,
  "test_end_acc": 0.671,
  "test_span_acc": 0.556,
  "test_per_instance_em": 0.613,
  "test_per_instance_f1": 0.7089842268487764,
  "training_duration": "0:03:42.210231",
  "epoch": 4,
  "training_start_acc": 0.979,
  "training_end_acc": 0.917,
  "training_span_acc": 0.905,
  "training_loss": 0.20337949429374438,
  "training_worker_0_memory_MB": 0.0,
  "training_gpu_0_memory_MB": 3234.48095703125,
  "validation_start_acc": 0.57,
  "validation_end_acc": 0.531,
  "validation_span_acc": 0.438,
  "validation_per_instance_em": 0.553,
  "validation_per_instance_f1": 0.6355119181646132,
  "validation_loss": 2.0518209609650073,
  "best_validation_start_acc": 0.57,
  "best_validation_end_acc": 0.531,
  "best_validation_span_acc": 0.438,
  "best_validation_per_instance_em": 0.553,
  "best_validation_per_instance_f1": 0.6355119181646132,
  "best_validation_loss": 2.0518209609650073
}
% 80% skip
Metrics: {
  "best_epoch": 3,
  "untrained_test_start_acc": 0.011,
  "untrained_test_end_acc": 0.008,
  "untrained_test_span_acc": 0.0,
  "untrained_test_per_instance_em": 0.0,
  "untrained_test_per_instance_f1": 0.03452869932892007,
  "peak_worker_0_memory_MB": 0,
  "peak_gpu_0_memory_MB": 3491.1279296875,
  "test_start_acc": 0.722,
  "test_end_acc": 0.737,
  "test_span_acc": 0.637,
  "test_per_instance_em": 0.705,
  "test_per_instance_f1": 0.7967874824320277,
  "training_duration": "0:04:05.548210",
  "epoch": 4,
  "training_start_acc": 0.844,
  "training_end_acc": 0.866,
  "training_span_acc": 0.768,
  "training_loss": 0.5212863344636317,
  "training_worker_0_memory_MB": 0.0,
  "training_gpu_0_memory_MB": 3491.1279296875,
  "validation_start_acc": 0.666,
  "validation_end_acc": 0.646,
  "validation_span_acc": 0.562,
  "validation_per_instance_em": 0.712,
  "validation_per_instance_f1": 0.7763576373639846,
  "validation_loss": 1.6714004439702257,
  "best_validation_start_acc": 0.664,
  "best_validation_end_acc": 0.647,
  "best_validation_span_acc": 0.563,
  "best_validation_per_instance_em": 0.71,
  "best_validation_per_instance_f1": 0.7765548149569085,
  "best_validation_loss": 1.6403362055178732
}
\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
         & Span accuracy & EM & F1 \\ \hline \hline
        $\mathcal{D}_{1}$ &0.59&0.66&0.79 \\ \hline
        % $\mathcal{D}_{u1}$ &0.53&0.2&0.68 \\ \hline
        $\mathcal{D}_{2}$ &0.69&0.75&0.86 \\ \hline
        $\mathcal{D}_{test}$ &0.68&0.74&0.83 \\ \hline
    \end{tabular}
    \caption{The RoBERTa has poor performance on the protected data $\mathcal{D}_{1}$, after fine-tuned on $\mathcal{D}_{u1} \cup \mathcal{D}_{2}$, where  $\mathcal{D}_{u1}$ is one version of $\mathcal{D}_{1}$ with a shortcut.}
    \label{tab:squad_partial}
\end{table}

Therefore, we assume that the effectiveness simply comes from the induced substitute words, which models may easily correlate with the labels during the training. 
We further hypothesize that \textbf{\textit{min-min optimization works by simply generating the noise containing explicit patterns to make the data unlearn rather than interact with each sample $x$. }}

% We also measure the accuracy for both starts and ends of answer spans. We find that the model can easily learn either starting or ending positions of training data (about 90\% accuracy) but cannot correctly locate the whole answer span (0 accuracy). 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{pics/dist-substitution-squad.png}
    \caption{The probabilities (i.e., normalized frequency) of substitution words. Only eight words generated via min-min optimization for all the 1000 training samples. Actually, the probability of the top-5 words is more that 98\%.}
    \label{fig:dist_sub_squad}
\end{figure}


\section{Related Work}
and how gradient-based methods are used for adversarial attacks, data poisoning and crafting unlearnable images.
\paragraph{Gradient-based methods.} 
Gradient-based methods have been shown effective to perturb data for different objectives. 
For example, \citet{ebrahimi2017hotflip,wallace2020imitation,wallace2019universal} generate adversarial examples by maximizing the cross-entropy loss of clean examples (error-max) \citep{goodfellow2014explaining},  while poison data are generated to maximize the loss of test data. Both attacks target the malicious behaviour of test data (min-max) \citep{munoz2017towards}. 

There are two specific gradient-based methods for word substitutions: (1) \citet{ebrahimi2017hotflip,wallace2019universal, wallace2021concealed} searched over potential substitutions via the first-order approximation. (2) \citet{behjati2019universal,cheng2020seq2sick} applied projected gradient descend to update continuous representations in the embedding space and perform projected operation for the textual input. In this paper, we use the first-order approximation for unlearnable objective.

Another example is data poisoning where attackers maliciously modify training texts to manipulate model behaviors at the inference time \citep{munoz2017towards, huang2020metapoison, kurita-etal-2020-weight, yang-etal-2021-careful, wallace2021concealed}.
% although the attack could be performed for the final models \citep{gu2017badnet}. 
% different
% Our work distinguishes from the poison attack since unlearnable text only prevents the learning rather than maliciously compromises the model performance or even manipulates model behaviours. Therefore, we minimize the training loss for the inner objective rather than maximize it.
% Also, \citet{wallace2021concealed, kurita-etal-2020-weight} constructs a backdoor attack (a type of poison attack) to make predictions of well-trained models manipulated by specific phrases (inference triggers) inserted into the text. To achieve this, they construct stealthy triggers for training different from inference triggers. Our class-wise unlearnable features are indeed overlapping triggers for both training time and inference time.

==> temp.tex <==
% manual experimental record
% SST LSTM M=30
% iteration, test accuracy
% 30, 0.73 
% 60, 0.78
% 90, 0.75

% AG-News LSTM M=30 ; Running time=14h
% iteration, test accuracy, orig test accuracy
% 0，0.26
% 30, 0.54 0.61
% 60, 0.75 
% 90, 0.64

% ToDo:
% merge generate_squad_unlearnable with generate_unleanable
% how to train? use generate_unleanable or use perturbed_data_reader or generate unlearnable texts



\subsection{How to Generate Shortcuts?} \label{sec:txt_mod}
\emph{  Word Insertion  }
To further verify that these explicit patterns can work without interaction with each samples

\begin{table*}
    \centering
    \centering
    \begin{tabular}{ |p{2cm}|p{1.8cm}|p{1cm}|p{1cm}|p{1cm}|p{1.5cm}|} 
     \toprule
     Task & Model & Orig & Min-min & Shortcuts & Untrained Accuracy\\
     \midrule
     \multirow{3}{*}{SST-2}
     & LSTM & 0.84 & 0.5 && 0.5  \\ \cline{2-6}
     & CNN & 0.83 & 0.5 && 0.5 \\ \cline{2-6}
     & BERT & 0.91 & 0.63 && 0.5 \\ \cline{2-6}
     \hline
     \multirow{3}{*}{AG-News}
     & LSTM & 0.91 && 0.35 & 0.25  \\ \cline{2-6}
     & CNN & 0.92 && 0.25 & 0.25 \\ \cline{2-6}
     & self-attention & 0.90 && 0.25 & 0.25\\ \cline{2-6}
     & BERT & 0.94 && 0.28 & 0.26 \\ \cline{2-6}
     \hline
     
     \multirow{2}{*}{SQuAD-1000}
     & BiDAF & 0.25 & 0.035 &&  0 \\ \cline{2-6}
     & RoBERTa & 0.73 & 0.024 && 0.01 \\ \cline{2-6}
     \hline
     
     \multirow{2}{*}{SQuAD}
     & BiDAF & 0.74 && 0.06 &  0.01 \\ \cline{2-6}
    %  0.74 for dev set
     & RoBERTa & 0.96 && 0.07 & 0.01 \\ \cline{2-6}
     
     \bottomrule
  \end{tabular}
    % \caption{Shortcuts.}{\small{We insert one class-wise character ('a', 'b', 'c', 'd' in the middle) for AG-News and a shortcut (a single number '2') in front of answer span for SQuAD.} }

    % \caption{The performance of DNNs trained on unlearanble text. We report accuracy on SST-2 and AG-News, and F1 scores for SQuAD. Modifications on BERT and RoBERTa are generated by surrogate models LSTM and BiDAF respectively. We show random/untrained accuracy to verify the unlearnability.}
\end{table*}
\section{Biased Features: Results and Analyses}
\paragraph{Evaluation.} We evaluate the following aspects to answer whether the shortcuts protect the data from being exploited during training:
(1) gradient norms during training: we expect that the model gradients always are zero as long as the shortcuts are embedded. ; (2) the accuracy of test samples with shortcuts; (3) the accuracy of test samples without shortcuts.
% We adjust the answer spans in the original data for word insertions to correctly compute the metrics.

\subsection{Text Classification}
% or data applied with class-wise triggers. We insert 'a' for male and 'b' for female in the middle of text. 
Specifically, we insert shortcuts into the users' descriptions.
% https://www.kaggle.com/sergioli212/predicting-authorship-corpus/edit
% topic-based sentiment analysis
% https://alt.qcri.org/semeval2016/task4/index.php?id=data-and-tools
According to previous findings, we add simple, class-wise triggers to the middle of their descriptions ('a' for male and 'b' for female).  compares the test accuracy during training on clean data or data with the class-wise triggers. Since the loss reaches convergence within one epoch of training, the test accuracy is measured after each update of model parameters. The simple, class-wise triggers successfully make the fine-tuning process of BERT-based classifier fail.  
% We also find the training acurracy reach 100\% within \? steps. 
% We also find that triggers with high PMI are more effective, the detailed result is shown in Appendix \ref{app:pmi}. \redcomment{Can we put Figure 7 in the main content?}
% \section{Triggers with High PMI}  \label{app:pmi}
% We assume that frequent words for each class can be more effective in real world. since even $\mathcal{D}_{clean}$ has such unlearnable cues, which reduce the demand for consciously constructing unlearnable text. However, we have to ensure that selected class-wise triggers are not common for another class. Therefore, we select triggers by considering both frequency and PMI for each class of the dataset. Figure \ref{fig:twitter} shows that the model was still updated when trained on data with random triggers, while triggers with high PMI result in nearly zero gradients during the whole training process.
% % \redcomment{Table \ref{} shows that with the same percentage of unlearnable text, triggers with high PMI require less percentage of unlearnable data.}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pics/pmi.png}
%     \caption{Gradient norm during the training of Gender Prediction on Twitter data.}
%     \label{fig:grad_norm_twitter}
% \end{figure}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
          Begin & Middle & End \\
        \hline
        \hline
          0.508 & 0.5 & 0.501 \\
         \hline
        % Triggers: 'disciplined' (pos); 'failing' (neg)
    \end{tabular}
    \caption{Positions of trigger insertion. The result is acquired during fine-tuning BERT on SST-2.}
    \label{tab:position-sst}
\end{table}

\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
          & Clean & Begin & Middle & End \\
        \hline
        \hline
         CNN    & 0.91 & 0.25 & 0.28 & 0.26 \\
         LSTM   & 0.92 & 0.35 & 0.25 & 0.23  \\
 Self-attention & 0.90 & 0.25 & 0.25 & 0.26 \\
         \hline
    
    \end{tabular}
    \caption{Effectiveness of different posistions. The results are evaluated on AG\_News for topic classification. All three neural nets are trained from scratch.}
    \label{tab:position-agnews}
\end{table}

Since our algorithm exposes class-wise patterns for unlearnability, we consider the operation of insertion so that we can avoid the risk of substituting important words, which are not detected by our constraints. We also study whether the end of samples would cause better unlearnability by inserting substitution words at different positions. Tables \ref{tab:position-agnews} and \ref{tab:position-sst} reveal that inserting words at all the positions can be effective. Since they are position-agnostic, in practice, adding them in the middle of each text can make them more invisible.

We use inserting class-wise, small characters into the middle of text as shortcuts: extremely simple triggers ('a' for positive class and 'b' for negative class) for SST-2, the AG-news during fine-tuning BERT. Both optimized triggers and randomly selected class-wise triggers achieve untrained accuracy (~50\%). 
We present the effectiveness on Table \ref{tab:result}.
% My Unproved or Wrong assumptions
% 1. effect of random parameters when $M$ is too small: experiment on large $M$ or update after achieving certain accuracy
% 2. superficial features from the initial batches before the first updating
% 3. prone to bias to specific tokens which gives low loss, especially. 
% 4. \redcomment{improve the effectiveness when using partial training examples: using loss ranking; focus on "not failing" }
% 5. Can adversarial training removes the effectiveness of unlearnable text?
% 6. \paragraph{Effect of data splits.} Sentiment classifiers for movie reviews could become unlearnable if amounts of reviews of a specific movie contain the movie name. This discourages splitting reviews of the same movie into training sets, which is indeed a common practice to prevent learners to memorize the association between movies and words unique to the movie, such as the IMDB splits with disjoint sets of movies \citep{andrew-2011-imdb}. It is important to re-consider the data split \citep{gorman-bedrick-2019-need}.
% 7. Task-specific strategy: insert words with high sentiment indications for each class: "triggers":  {"0": ["2-faces"], "1": ["a+"]}

We instantiate biased features by the position and a token in the vocabulary, i.e., $b=(p, s)$. 

Since the model only cannot learn any other information from the text $x$ after achieving the highly unlearnable state, we expect that shortcuts should be as "short" as possible. 
In other word, the biases should easily correlate to the labels, i.e., $b \rightarrow y$. To achieve this goal, we build an optimization process to generate unlearnable biases.

To simplify the process, we only instantiate $\Phi$ as text modifications. We aim to find word substitutions for the inner objective \ref{eq:unlearnable}. Formally, we optimize unlearnable modification $(p, s)$ where the position $p$ informs where to modify and the substitution $s$ suggests what to modify.

\subsection{Question Answering}

We design several experiments to verify this hypothesis, we (1) fix substitutions as "the", which achieves the very similar effectiveness; (2) randomly select the modification positions $P$ excluding the answer spans, which barely has no effectiveness. Both results support our assumption; (3) We add substitution words (e.g., 'product') to arbitrary positions of test examples and find that the models trained/fine-tuned on unlearnable texts always predict phrases surrounding substitution word as answers, which further verifies the hypothesis.

% Other experiments
% (1) Suggested by Ma: Following this finding, we also investigate \redcomment{whether such shortcuts exist during the normal training process by removing surrounding words of correct answers (we choose examples which have stopwords surrounding answers so that removing stopwords would not affect text semantics.). -> There is no degrade of performance on fine-tuned transformer QA.} 
% (2) Manually constructed, random shortcut words before the answer spans instead of substitutions


\begin{table}[ht!]
    \centering
    \begin{tabular}{|p{1.7cm}|p{1.3cm}|p{1.1cm}|p{1.1cm}|}
        \hline
        & \parbox{1.3cm}{Span \\Accuracy} & EM & F1 \\
        \hline \hline
        Min-min & 0.012  &  0.023 & 0.035 \\
        \hline
        Fixed $S$ & 0.006  & 0.011 & 0.038 \\
        \hline
        Random $P$ & 0.58  &  0.61 & 0.72 \\
        \hline
    \end{tabular}
    \caption{Evaluating the importance of substitutions and position for min-min modifications. The table reports metrics on test data when we fix substitutions to one word or select random positions to modify. It shows that the modifications are effective as long as we put common substitution word(s) surrounding answers.}
    \label{tab:fixedS_randomP}
\end{table}


Finally, we use the hypothesis on the whole SQuAD training set by simply inserting the shortcut word "2" in front of answers. The result in Table \ref{tab:result} shows the effectiveness of unlearnable text.
% \section{The Unlearnable Hypothesis }

==> text_gen.tex <==
\section{Unlearnable Text for Generation}
Text summarization is a significant task in many domains, such as media monitoring \citep{nallapati-etal-2016-abstractive} and summarizing scientific \citep{chandrasekaran2020overview,ju-etal-2020-monash} documents. Unlike classification tasks labelled with finite classes for outputs, generation models output infinite combinations of tokens and have no explicit decision boundary for the class-wise settings.

\paragraph{Dataset.} We select CNN/Daily Mail and Xsum datasets. The former has highly abstractive summaries while the latter summaries resemble the source sentences \citep{lewis-etal-2020-bart}.

\begin{itemize}
    \item CNN/DM Mail corpus for summarization: The dataset constains long (hundreds of words) news articles and manually crafted multi-sentence summaries. It includes 286,817 training samples, 13,368 validation samples and 11,487 test samples. We down-sample 3000 article-summary pairs for training and use the first 1000 samples for validation.
    \item Xsum 
\end{itemize}
% 
% "The source documents in the training set have 766 words spanning 29.74 sentences on an average while the summaries consist of 53 words and 3.72 sentences."

\paragraph{Models.} We use both the LSTM encoder-decoder model with additive attention \citep{bahdanau-2015-attention}, BART \citep{lewis-etal-2020-bart} and GPT-2 \citep{radford2019language}. Both BART and GPT-2 are transformer-based, pre-trained models. However, BART uses encoder-decoder architecture while GPT-2 leverages only the decoder segment of transformer. 

\paragraph{Evaluation.} We report ROUGE scores. Although the N-gram overlap metrics are not as good as human evaluation for text summarization, it can reflect the worse performance of models trained on the unlearnable data compared to the well-trained models.

\begin{itemize}
    \item LSTM encoder-decoder: We try to re-implement the model by \citet{rush-etal-2015-neural}. It consists of two-layer, bi-directional LSTM for the attention based encoder and another two-layer LSTM for the decoder with hidden size 1000. We train the LSTM encoder-decoder with a minibatch SGD algorithm with Adadelta optimizer, learning rate 0.05, batch size 16 and each minibtach grouped by input length (Bucket sampler). 
    \item BART : It has 6 encoder and 6 decoder layers, with a hidden size of 768. We use a shared embedding layer for both the encoder and decoder. They are fine-tuned by Adam with weight decay, learning rate 3e-5.
    % the Rouge-1/2/L score:
    % original fairseq implementation -> 44.16/21.28/40.90
    % allennlp implementation -> 
    \item GPT-2: Unlike previous two models, it is essentially a casual language model, which only consists of 6 decoder layers. 
    % training and inference
    Same as BART, the decoder attention mask allows one forward pass for predicting all the target tokens during fine-tuning while the decoding process during inference would be performed regressively by involving previous predictions.
    % delimiter
    To accommodate the auto-regressive model for text summarization, we follow the original setup \citep{Radford2018ImprovingLU,khandelwal2019sample} and add a delimiter to concatenate the article and summary and a padding token for training. 
    % max_length
    We only select samples whose concatenated, tokenized text has the maximum length 1024 due to the constraint of the GPT-2 model.
    % small (117M parameters) , medium (345M parameters), large (774M parameters) and XL (1.5B parameters)
\end{itemize}

\subsection{Experimental Result}

\paragraph{The last word is significant for LSTM enc-dec.} With attention mechanism, the context vector is calculated as the weighted sum of all the input sequences. However, still

\paragraph{Unlearnable patterns learn from LSTM enc-dec are effective on auto-regressive models (GPT-2)?}

\paragraph{Different decoding algorithms.} To ensure the unlearnable effectiveness, we evaluate the metrics with different decoding algorthms and all of them show poor performance.

\paragraph{Vocabulary.} Unseen words in validation data result in OOV placeholders for both predictions and reference sentences. The vocabulary is constructed by both training and validation set.

% Beam search implementaiton:
% -> transformer/fairseq
%    take the sequence with the highest *average* of log probability per token
%    with length penalty
% -> AllenNLP
%    take the sequence with the highest   *sum*   of log probability per token 


